Oblivious Online Contention Resolution Schemes

Contention resolution schemes (CRSs) are powerful tools for obtaining "ex post feasible" solutions from candidates that are drawn from "ex ante feasible" distributions. Online contention resolution schemes (OCRSs), the online version, have found myriad applications in Bayesian and stochastic problems, such as prophet inequalities and stochastic probing. When the ex ante distribution is unknown, it was unknown whether good CRSs/OCRSs exist with no sample (in which case the scheme is oblivious) or few samples from the distribution. In this work, we give a simple $\frac{1}{e}$-selectable oblivious single item OCRS by mixing two simple schemes evenly, and show, via a Ramsey theory argument, that it is optimal. On the negative side, we show that no CRS or OCRS with $O(1)$ samples can be $\Omega(1)$-balanced/selectable (i.e., preserve every active candidate with a constant probability) for graphic or transversal matroids.

==> exchange.tex <==
\subsection{Proof of Lemma~\ref{lemma:prophet_competitive_ratio}}
\label{subsec:bases_exchange}

Observe that we select items in a conservative way, in the sense that $\Prx{i \text{ is active} \mid v_i =v} \le \Prx{i \in \opt \mid v_i=v}$ for all $i,v$. 
Nevertheless, we prove that the expected values of the active items are $\epsilon$-close to the optimum.

Before that, we prove the following monotone basis exchange lemma for matroids. 

\begin{lemma}
	\label{lemma:monotone_mapping}
	Let $\matroid = (U, \indset)$ be a weighted matroid with weight function $w: U \rightarrow \mathbb{R}_{\ge 0}$. Suppose $A \in \mathcal{I}$ is the basis with maximum total weight. For every basis $B$, there exists a bijection $f: A \rightarrow B$ such that for all $x \in A$, $B - f(x) + x$ is a basis and $w(f(x)) \leq w(x)$. 
	Moreover, the bijection $f$ satisfies that $f(x) = x$ for all $x \in A \cap B$. 
\end{lemma}

It is worthwhile to make a comparison to the following lemma in the literature. 

\begin{lemma}[Lemma 1, Section 3.3 of \cite{KW19}] \label{lemma:mapping_easy}
	Let $\matroid = (U, \indset)$ be a weighted matroid with weight function $w: U \rightarrow \mathbb{R}_{\ge 0}$. Suppose $A \in \indset$ is the basis with maximum total weight. For every basis $B$, there exists a bijection $g: B \rightarrow A$ such that for all $y \in B$, $A - g(y) + y$ is a basis and $w(g(y)) \geq w(y)$. 
\end{lemma}

Observe that the only difference between the two lemmas is the direction of the mappings $f,g$. We argue that our lemma is more difficult since for every bijection $g$ such that $A-g(y)+y$ is a basis, we must have $w(g(y)) \geq w(y)$ as otherwise $w(A - g(y) + y) > w(A)$. In contrast, our lemma does not hold for every bijection $f$ such that $B-f(x)+x$ is a basis.
%But Lemma \ref{lemma:strong_exchange} is far from obvious, and it may be surprising that it actually holds. 

\paragraph{Proof of Lemma~\ref{lemma:monotone_mapping}} 
Let $U = [n]$ and $w(1) \geq w(2) \geq \cdots \geq w(n)$. Suppose the rank of the matroid is $r$. We denote the elements in $A$ by $\{a_i\}_{i \in [r]}$ where $a_i$'s are in ascending order. Consequently, we have $w(a_1) \ge w(a_2) \ge \cdots \geq w(a_r)$. Without loss of generality, we can assume that the basis $A$ is generated by feeding $1, 2, \cdots, n$ to the greedy algorithm sequentially.


Next, we state our algorithm for constructing the bijection $f$. We will need the strong basis exchange property stated in Lemma~\ref{lemma:strong_exchange}. 

\begin{algorithm}[H]
	\SetAlgoLined
	\caption{Construct mapping $f$}
	\label{alg:mapping}
	{Recall $r$ is the rank of $\matroid$}
	
	{$A_{r + 1} \gets A$}
	
	\For{$i \gets$ $r, r - 1, \cdots, 1$ in descending order}{
		\If {$a_i \in A_{i + 1} \setminus B$} {
			{By Lemma \ref{lemma:strong_exchange}, there is an element $b_i \in B \setminus A_{i + 1}$ such that $A_{i + 1} - a_i + b_i$ and $B - b_i + a_i$ are both bases.}
			
			{Let $f(a_i) \gets b_i$}
			
			{$A_i \gets A_{i + 1} - a_i + f(a_i)$}
		}
		\Else {
			{Let $f(a_i) \gets a_i$}
			
			{$A_i \gets A_{i + 1}$}
		}
	}
\end{algorithm}

We first prove the following facts about Algorithm \ref{alg:mapping}. 

\begin{fact} \label{fact:subset}
	$\{f(a_i), f(a_{i + 1}), \dots, f(a_r)\} \subset A_i$. 
\end{fact} 
\begin{proof}
	For all $j \geq i$, if $a_j \in A_{j + 1} \setminus B$, we have $f(a_j) \in B \setminus A_{j + 1}$ which implies $f(a_j) \not\in \{a_i, \dots, a_j\}$. Together with $f(a_j) \in A_j$, we can see that $f(a_j)$ is never eliminated and $f(a_j) \in A_i$. If $a_j \not\in A_{j + 1} \setminus B$, we know $f(a_j) = a_j$, and it is in both $A_j$ and $A_i$. 
\end{proof}

\begin{fact} \label{fact:bijection}
	The resulting mapping $f$ is a bijection. 
\end{fact} 
\begin{proof}
	If $a_i \in A_{i + 1} \setminus B$, since $b_i \in B \setminus A_{i + 1}$, we know $f(a_i) = b_i \not\in \{f(a_{i + 1}), \dots, f(a_r)\}$ (by Fact \ref{fact:subset}). If $a_i \not\in A_{i + 1} \setminus B$, $f(a_i)$ equals $a_i$ itself. Note for all $j > i$, $A_{j + 1} - a_j + f(a_j)$ is a basis and $a_i \in A_{j + 1}$. Therefore $f(a_i) = a_i$ cannot equal to any of such $f(a_j)$. 
	
	Thus $f(a_i) \not= f(a_j)$ for all $j > i$. $f$ is an injection. Since $A$ and $B$ are two bases and $|A| = |B|$, $f$ is a bijection. 
\end{proof}

\begin{fact} \label{fact:monotone}
	For all $a_i \in A$, $w(f(a_i)) \leq w(a_i)$. 
\end{fact}
\begin{proof}
	If $w(f(a_i)) > w(a_i)$, we know $f(a_i) < a_i$. Thus $f(a_i)$ is fed to the greedy algorithm before $a_i$. 
	On the other hand, since $f(a_i) \ne a_i$, we must have $a_i \in A_{i + 1} \setminus B$ and $A_{i + 1} - a_i + f(a_i)$ is a basis. Therefore $\{a_1, a_2, \dots, a_{i - 1}, f(a_i)\} \in \indset$. Then our greedy algorithm should have selected $f(a_i)$ before it selected $a_i$. Since we enumerate $a_i$ in decreasing order of their index, if our algorithm selected $f(a_i)$, we must have $f(a_i) \in A_{i + 1}$. This contradicts with the fact $f(a_i) \in B \setminus A_{i + 1}$. 
\end{proof}

Finally, we verify that for all $a_i$, $B - f(a_i) + a_i$ is a basis. It is trivial when $f(a_i) = a_i$. Otherwise, $B - f(a_i) + a_i$ is also a basis according to our construction. This finishes the proof of the lemma.
\qed

\medskip

Now, we are ready to prove Lemma~\ref{lemma:prophet_competitive_ratio}.
The crucial part is to bound the contribution of those items with $\vali < T_0^i$.

\begin{lemma}\label{lemma:prophet_small_values}
	If $\{T_k^i\}$ are good thresholds, 
	\[
	\E{\sum_{i\in\OPT}\vali \cdot \I{\vali < T_0^i}} \le O(\epsilon) \cdot \E{\opt}.
	\]
\end{lemma}

\begin{proof}
	Let $W=\argmax_{S\in\indset}\sum_{i\in S} T_0^i$ be the maximum weighted basis where item $i$ has value $T_0^i$.
	Fix arbitrary $\vals$ and $\OPT(\vals)$, by Lemma \ref{lemma:monotone_mapping}, there exists a bijection $f: W \rightarrow \OPT$ such that for any $j \in W$, $\OPT-f(j) + j \in \indset$ and $T_0^{f(j)} \le T_0^j$. Moreover, for all $j \in W \cap \OPT$, $f(j) = j$. 
	
	By Observation~\ref{obs:is_threshold}, for every $j \in W \cap \OPT$, we have $f(j)=j$ and $\vali[j] \ge \tau_j(\valsmi[j])$. For every $j \in W \setminus \OPT$, by Observation \ref{obs:tau_property}, we also have $\vali[f(j)] \ge \tau_j(\valsmi[j])$.
	Hence, $\vali[f(j)] \ge \tau_j$ for all $j \in U$. Consequently,
	\begin{equation}
	\Prx{\vali[f(j)] \ge T_0^j} \ge \Prx{\tau_j(\valsmi[j]) \ge T_0^j} \ge 1- \epsilon - \epsilon^2, \label{eqn:prob}
	\end{equation}
	where the last inequality holds when $\{T_k^i\}$ are good.
%	for every $j \in W$, which also implies $\Prx{\vali[f(j)] < \widehat{T}_{j,0}} \le \epsilon + \epsilon^2$.
	Then, 
	\begin{equation}
	\E{\sum_{i\in\OPT}\vali} = \E{\sum_{j \in W} \vali[f(j)]} \ge \E{\sum_{j\in W} T_0^j \cdot \I{\vali[f(j)] \ge T_0^j}} \ge (1-\epsilon-\epsilon^2)\sum_{j\in W} T_0^j. \label{eqn:lowerbound}
	\end{equation}
	Recall that by the construction of $f$, we have that $T_0^{f(j)} \le T_0^{j}$, $\forall j \in W$. Equivalently, we have $T_0^{f^{\text{-}1}(i)} \ge T_0^i$, $\forall i \in \OPT$. Finally,
	\begin{align*}
	\E{\sum_{i\in\OPT}\vali \I{\vali < T_0^i}} \le{} & \E{\sum_{i\in\OPT}\vali \I{\vali < T_0^{f^{\text{-}1}(i)}}} \le \E{\sum_{i\in\OPT}T_0^{f^{\text{-}1}(i)} \I{\vali < T_0^{f^{-1}(i)}}}\\
	={} & \E{\sum_{j\in W} T_0^j \I{\vali[f(j)] < T_0^j}} \stackrel{\eqref{eqn:prob}}{\le} (\epsilon+\epsilon^2) \sum_{j\in W} T_0^j \\
	\stackrel{\eqref{eqn:lowerbound}}{\le}{} & \frac{\epsilon+\epsilon^2}{1-\epsilon-\epsilon^2} \E{\opt} \le O(\epsilon) \cdot \E{\opt}. 
	\qedhere
	\end{align*}
\end{proof}

\paragraph*{Proof of Lemma~\ref{lemma:prophet_competitive_ratio}}

For every $i \in U$ and $v \in [T_k^i,T_{k+1}^i)$, we have 
\begin{align*}
p^i(v) \le p^i(T_{k+1}^i) \le{} & \epsilon(1+\epsilon)^{k+1} + \epsilon^2 & \mbox{since $\{T_{k}^i\}$ are good} \\
\le{} & (1+O(\epsilon)) \cdot (\epsilon(1+\epsilon)^k - \epsilon^2) \\
={} & (1+O(\epsilon)) \Prx{i \in R(\allocs) \mid \vali=v}. & \mbox{by the activation rule}
\end{align*}
Therefore,
\begin{align*}
\E{\sum_{i \in \OPT} \vali \I{\vali \ge T_0^i}} ={} & \sum_{i \in [n]} \int_{T_0^i}^{\infty} v p^i(v) \dd F_i(v) \\ 
\le{} & (1+O(\epsilon)) \sum_{i \in [n]} \int_{T_0^i}^{\infty} v \Prx{i \in R(\allocs) \mid v_i = v} \dd F_i(v) \\ 
={} & (1 + O(\epsilon))\E{\sum_{i \in R(\allocs)} \vali}.
\end{align*}

Combine this inequality with Lemma~\ref{lemma:prophet_small_values}, we conclude that
\begin{align*}
\E{\sum_{i\in R(\allocs)}\vali} \ge{} & \frac{1}{1+O(\epsilon)} \E{\sum_{i\in\OPT}\vali\I{\vali\ge T_0^i}} \\
={} & \frac{1}{1+O(\epsilon)} \left(\E{\opt} - \E{\sum_{i\in\OPT}\vali\I{\vali < T_0^i}} \right) \ge \frac{1}{1+O(\epsilon)} \E{\opt}.
\end{align*}
\qed


==> laminar.tex <==
% We first recall the definition of laminar matroids.
% A set family $\mathcal{L}\subseteq 2^U$ is \emph{laminar} if for two sets $A,B \in \mathcal{L}$, either $A \cap B = \emptyset$, or $A \subseteq B$ or $B \subseteq A$. 
% A \emph{laminar matroid} is defined by a laminar family $\mathcal{L}$ and a set of positive integers $\{r_L\}_{L\in \mathcal{L}}$; a set $A\subseteq U$ is independent if and only if $|A\cap L|\leq r_L$ for all $L \in \mathcal{L}$. 

% Observe that we can safely assume a few things about the numbers $r_L$: \begin{itemize}
    % \item $r_L \leq |L|$ for every $L \in \mathcal L$: if not, the restriction $|A\cap L|\leq r_L$ is redundant. 
    % \item $r_L \leq r_M$ for any $L\subset M$: if not, the restriction $|A\cap L|\leq r_L$ is redundant.    
% \end{itemize} 
% The matroid polytope of a laminar matroid defined by the laminar family $\mathcal{L}$ and values $\{r_L\}_{L\in \mathcal{L}}$ is:
% $$\mathcal{P}=\{\allocs\in [0,1]^U \ : \ \sum_{i\in L} x_i \leq r_L, \ \forall L\in \mathcal{L}\}.$$

% Consider the following simple algorithm, parameterized by a constant $b \in [0, 1]$ to be fixed later: \\
% \begin{algorithm}[H]
% \SetAlgoLined
% $S \gets \emptyset$ \\
 % \For{ each arriving $i\in U$}{
 % \If {$i$ is active and $S+i\in \mathcal{I}$}
  % {Add $i$ to $S$ w.p. $b$}
 % }
 % \Return $S$
 % \caption{An oblivious OCRS for matroids.}
% \label{alg:laminar}
% \end{algorithm}
% Algorithm~\ref{alg:laminar} is almost greedy, except that w.p. $1-b$ it rejects active elements that it could accept. 
% We can interpret it as running the greedy algorithm on the random set $R(b\allocs)$. 

In this section, we show that the $b$-Greedy OCRS is $\Omega(1)$-selectable for laminar matroids.

We first recall the definition of laminar matroids.
A set family $\mathcal{L}\subseteq 2^U$ is \emph{laminar} if for any $A,B \in \mathcal{L}$, either $A \cap B = \emptyset$, or $A \subseteq B$ or $B \subseteq A$. 
A \emph{laminar matroid} is defined by a laminar family $\mathcal{L}$ and a set of positive integers $\{r_L\}_{L\in \mathcal{L}}$; a set $A\subseteq U$ is independent if and only if $|A\cap L|\leq r_L$ for all $L \in \mathcal{L}$. 
Without loss of generality, we may assume $r_L \leq |L|$ for every $L \in \mathcal L$, and $r_L < r_M$ for every $L$ that is a proper subset of $M$.
The polytope of a laminar matroid defined by the laminar family $\mathcal{L}$ and values $\{r_L\}_{L\in \mathcal{L}}$ is
$\mathcal{P}=\{\allocs\in [0,1]^U \ : \ \sum_{i\in L} x_i \leq r_L, \ \forall L\in \mathcal{L}\}$.

\begin{theorem}
% Algorithm~\ref{alg:laminar} 
The $b$-Greedy OCRS is oblivious and $0.0715$-selectable on any laminar matroid for $b=0.13$.
\end{theorem}

\begin{proof}
Consider an arbitrary element $i\in U$ and let $L_1\subset L_2 \subset \ldots \subset L_k$ be the maximal chain in $\mathcal{L}$ that contains $i$.
Note that, since $\mathcal{L}$ is laminar, $L_1, \cdots, L_k$ are all the sets in $\mathcal{L}$ that contain~$i$.
For ease of notation, define $r_j:=r_{L_j}$. 
% Since $L_j$ is a proper subset of $L_{j+1}$, by our assumption w.l.o.g. 
Without loss of generality, we may assume $r_j < r_{j + 1}$. (Otherwise, removing $L_j$ from~$\mathcal L$ and the constraint $\sum_{i \in L_j} \alloci \leq r_j$ leaves the matroid remaining the same.)
Recall that $R(\allocs)$ denotes the random set of active items.
Since the $b$-Greedy OCRS accepts any selectable element with probability~$b$, it is equivalent to view it as running the ($1$-)Greedy OCRS on a set of active elements drawn from distributions given by~$b\allocs$.  
We have 
%\Hongxun{Maybe we should explain what $R(b\allocs)$ is.}
    \begin{align*}
    \Prx{i \text{ is selected} \mid \text{$i$ is active}} 
    % &\geq \Prx{i\in R(b \allocs)
    % \text{ and } 
    % \wedge |(R(b\allocs)\cap L_j)-i|< r_j, \ \forall j\in [k]}\\
    &\geq b \Prx{|(R(b\allocs)\cap L_j)\setminus \{i\}|< r_j, \ \forall j\in [k]} \\
    % & \text{by independence} \\
    % &= bx_i \left(1-\Prx {\bigcup_{j\in [k]} |(R(b\allocs)\cap L_j)-i|\geq r_j}\right) \\
    &\geq b \left(1-\sum_{j\in [k]} \Prx{|(R(b\allocs)\cap L_j) \setminus \{i\}|\geq r_j}  \right),
    \end{align*}
    where the last inequality follows from the union bound.
    Since $\allocs$ is in the matroid polytope, we have $\sum_{i' \in L_j} \alloci[i'] \leq r_j$.
    Therefore each summand on the right hand side can be bounded by the Chernoff bound:
    % & \text{by union bound}\\
    \begin{align*}
    \Prx{|(R(b\allocs)\cap L_j) \setminus \{i\}|\geq r_j} 
    %&\leq bx_i \left( 1- \sum_{j\in [k]} 
    \leq \left( \frac{\exp((1-b)/b)}{(1/b)^{(1/b)}} \right)^{br_j}.
    %\right)
    % & \text{by Chernoff bound}\\
    \end{align*}
    We can now see that the sum of probabilities in the bound above converges to a constant that depends on~$b$:
    \begin{align*}
    \Prx{i \text{ is selected}\mid \text{$i$ is active}} 
    &\geq b \left(1- \sum_{j\in [k]}(b \exp(1-b))^{r_j} \right)  \geq b \left(1- \sum_{j=1}^{\infty}(b \exp(1-b))^j \right) \\ 
    % & \text{since } r_{j}<r_{j+1}\\
    &= b \left(1-\frac{be^{(1-b)}}{1-be^{(1-b)}}\right).
    \end{align*}
    In the second inequality we used $r_j < r_{j+1}$. 
% We use the fact that $x$ belongs to the matroid polytope to apply the Chernoff bound. 
With $b$ chosen to be $0.13$, the right hand side is at least $0.0715$.
% we obtain a $0.0715$-selectable OCRS. 
\end{proof}
\begin{observation}
Contention resolution when the elements arrive in a uniformly random order has also been studied in the literature \cite{AW18, LS18}, and the algorithms are called \emph{Random order Contention Resolution Schemes} (RCRS).  
Our analysis also yields an oblivious RCRS with a slightly better selectability when $b$ is appropriately chosen.
%If the elements arrive in random order, we can just use the same algorithm with another $b$ to get a better result. 
% The only difference in the analysis is that, 
The analysis needs a slight change:
to be able to accept element~$i$, 
% instead of requiring $|(R(b\allocs)\cap L_j) \setminus \{i\}|< r_j \ \forall j\in [k]$, 
we need $|R(b\allocs)\cap B(i)\cap L_j|< r_j$ for all $j\in [k]$, where $B(i)$ is the random set of elements that arrive before $i$;
with random arrival order, each element in $U-\{i\}$ belongs to $B(i)$ independently with probability~$\tfrac 1 2$. 
So $\Ex{|(R(bx)\cap B(i)\cap L_j)|}$ is upper bounded by $br_j/2$. 
This improves the Chernoff bound. 
% By basically the same calculation and taking 
An analysis similar to the above with $b=1/4$ gives a $0.142$-selectable RCRS.
\end{observation}

\begin{observation}
A uniform rank~$r$ matroid ($I\in \mathcal{I}$ iff $|I|\leq k$) is a special case of laminar matroid ($\mathcal{L}=\{U\}$ and $r_U=r$). 
% We can use the same algorithm, but simplify the analysis and pick a different $b$ (as function of $r$) to get an 
But in this case we can simplify the analysis and show that, as $r$ goes to infinity, the $b$-Greedy algorithm has selectability arbitrarily close to~$1$, with appropriately chosen~$b$.  
% To simplify the analysis, 
More specifically, we know that the maximal chain is simply $U$ in this case, so we no longer need the union bound and we get $$\Prx{i \text{ is selected} \mid \text{$i$ is active}}\geq b(1-(b\exp(1-b))^r).$$ 
Note that for any fixed $b\in (0,1)$, $\displaystyle \lim_{r\rightarrow \infty} b(1-(b\exp(1-b))^r)=b$. So for any $b\in (0,1)$, $\epsilon>0$, $\exists r_0 \in \N$ such that $b$-Greedy is $(b-\epsilon)$-selectable for any uniform rank $r$ matroid with $r\geq r_0$.   
\end{observation}















==> matroid_prophet.tex <==
In this section, we study the sample-based matroid prophet inequality problem and obtain a constant competitive algorithm via the OCRS approach. 

We first review the standard OCRS approach for tackling prophet inequalities in the full information setting and then highlight the challenges in the sample-based setting. The matroid prophet inequality problem can be solved by the following three steps.
\begin{itemize}
	\item Calculate the random vector $\allocs$ where $\alloci = \Prx{i \in \opt}$ and the corresponding OCRS $A$ of $\allocs$.
	\item Upon the arrival of an item $i$ with value $\vali$, resample $\widehat{\valsmi} \sim \times_{j \ne i}F_{j}$ and compute the optimal solution $\opt'$ with respect to $(\vali,\widehat{\valsmi})$.
	\item Consider $i$ being active if and only if $i\in \opt'$ and then apply $A$.
\end{itemize}

%\Hongxun{Changed $\opt_i$ to $\opt'$ to avoid confusion with $\opt_i$ in 4.1}

It is shown that the above algorithm transfers any $c$-selectable OCRS to a $c$-competitive algorithm for the matroid prophet inequality.
However, it is not clear how to adapt the approach to the sample-based setting, if we restrict ourselves to $O(\log n)$ number of samples. We explain in detail the difficulties we will encounter if we straightforwardly follow the above algorithm.
\begin{itemize}
    \item First of all, we need to construct an OCRS with respect to the vector $\allocs$ where $\alloci = \Prx{i \in \opt}$. Though we have shown that $O(\log n)$ number of samples are enough to learn a constant selectable OCRS, it is not clear how we generate $R(\allocs)$ with value samples. If we simply compute the optimal solution from a value sample $\vals$, each item $i$ would be active with the right marginal probability $\alloci$ but fails to be active independently. Recall that $R(\allocs)$ requires independence across different items.
    \item More crucially, upon the arrival of an item, we have to determine whether it is active or not. To use the resampling approach, we would need for each item a fresh sample from $\times F_i$, that leads to $\Omega(n)$ number of samples.
\end{itemize}

To resolve the issues, one might come up with the idea of learning a set of thresholds $\{\tau_i\}$ and considering each item as active \emph{iff} $\vali \ge \tau_i$. Indeed, if we are able to learn the thresholds accurately such that $\Prx{v_i \ge \tau_i} = \Prx{i \in \opt}$, we are effectively solving the \emph{ex-ante} relaxation of the problem and could then apply the corresponding OCRS. Unfortunately, in the sample-based setting, we could only approximate the vector $\allocs$ up to $\epsilon$ accuracy and it is unclear how should we set the thresholds. For instance, if our algorithm accepts items in an aggressive way (i.e. set low thresholds), the corresponding vector $\allocs$ of our algorithm would be out of the matroid polytope; if our algorithm accepts items in a conservative way (i.e. set high thresholds), we might have given away a large fraction of the optimal.

%Consider the case when each item has some large value with probability $\frac{1}{n}$ and $0$ otherwise. With only $o(n)$ samples, for each item $i$, it is high probability that all the sample values of $i$ equal $0$, in which case we have no idea on how to set $\tau_i$. 
We circumvent these difficulties in a highly non-trivial way. Below, we summarize our approach to offer more intuitions. The formal proof is in Section~\ref{subsec:prophet}.
\begin{itemize}
    \item Instead of learning a single threshold for each item, we try to learn the function $p^i(v) \eqdef \Prx{i \in \opt \mid \vali = v}$. Observe that this function only depends on the distributions $\{F_j\}_{j \ne i}$. In contrast, the threshold $\tau_i$ discussed above relies on the distribution of $F_i$ as well.
    
    Informally, we discretize the quantile space $[0,1]$ into a sequence of constants $\{p_k\}$, where $p_k$'s are defined according to the accuracy parameter $\epsilon$.
	We learn with high probability a set of good thresholds $\{T_{k}^{i}\}_{k=0}^m$ such that if $v_i \in [T_k^i, T_{k+1}^i)$, then $p^i(v_i) \in [p_k, p_{k+1} + 2\epsilon^2]$. \footnote{The $2\epsilon^2$ term here is the error bar for concentration, and will be clear later.} This can be done with $O(\log n)$ number of samples by standard concentration arguments.
	\item Given the thresholds, we specify an \emph{activation rule} to determine whether an item $i$ is active. For $v_i \in [T_k^i, T_{k+1}^i)$, let $v_i$ be active with probability $p_k$. Consequently, this rule induces a way of transforming a value sample $\vals$ to a set sample from $R(\allocs)$, where $\alloci = \Prx{i \text{ is active}}$.  By the conservative nature of our algorithm, we prove that $\allocs$ is in the matroid polytope $\polytope_{\matroid}$.
	
	On the other hand, since we are running the algorithm in a conservative way, we unavoidably give away items with small values. We are left to show that the loss is not too significant. This is the most technically challenging part of our analysis. Our proof builds on a novel monotone basis exchange lemma for matroids, that might be of independent interests.
    \item Now we are equipped with a sample oracle of $R(\allocs)$ and we can apply Theorem~\ref{thm:matroid_ocrs} to construct an OCRS. Finally, in the real run of the prophet inequality, we use the activation rule to determine whether an item is active and then feed it to the OCRS to finish our algorithm.
\end{itemize}


%\zhihao{holding the token}
%In this section, we apply matroid OCRS with $O(\log n)$ samples to matroid prophet inequality, and obtained $\left(\frac{1}{4} - \epsilon\right)$-competitive matroid prophet inequality from $O(\log n)$ samples. On high level, our approach contains two steps:
%
%\begin{itemize}
%    \item From $O(\log n)$ samples, learn a set of thresholds. To be $\left(\frac{1}{4} - \epsilon\right)$-competitive, we actually need to learn more than one threshold for each item. For now, just assume we learn a single threshold $T_i$ for each item. 
%    \item Now we have already learned and fixed each $T_i$. For those items above its threshold, namely $v_i > T_i$, we view them as active. Since those $T_i$ are fixed, different items are independent in terms of being active. Then we apply matroid OCRS to pick active items. 
%\end{itemize}
%
%Note in this procedure, we ignored all the items with value $v_i$ below $T_i$. Thus we may incur a large cost. To prove this is not the case, we need a novel monotone basis exchange lemma for matroid together with a charging argument. From Theorem \ref{thm:non_existence_graphical} and Theorem \ref{thm:non_existence_transversal}, we know that there is no OCRS for general matroid from finite samples. Therefore, following this approach, one cannot get a finite sample matroid prophet inequality with constant gambler-to-prophet ratio. 

%Note in this procedure, we ignored all the items with value $v_i$ below $T_0^i$. Thus we may incur a large cost. To prove this is not the case, we need a novel monotone basis exchange lemma for matroid together with a charging argument. From Theorem \ref{thm:non_existence_graphical}, we know that there is no OCRS for general matroid from finite samples. Therefore, following this approach, one cannot get a finite sample matroid prophet inequality with constant gambler-to-prophet ratio. 


%This section is organized as follows: We first present the monotone basis exchange lemma in \ref{subsec:bases_exchange}. Then in \ref{subsec:prophet}, we introduce our algorithm and the charging argument. 

\input{prophet}

\input{exchange}


==> prelim.tex <==
\paragraph{Contention Resolution Schemes (CRS)}
Given a universe $U = [n]$, consider a matroid $\matroid = (U, \indset)$ where $\indset \subseteq 2^U$ is the set of independent sets and its polytope $\polytope_{\matroid} \coloneqq \{\allocs \in \mathbb [0, 1]^n \given \sum_{i \in S} \alloci \leq \rank(S), \forall S \subseteq U\}$.
A Contention Resolution Scheme (CRS) takes as input a vector $\allocs \in \polytope_\matroid$ and a random set $R(\allocs)$ where each element $i \in U$ is in $R(\allocs)$ with probability $\alloci$ independently; the CRS must then output an independent set $S \in \indset$ that is a subset of $R(\allocs)$.  
An element $i \in U$ is said to be \emph{active} if it appears in $R(\allocs)$.
A CRS is said to be \emph{$c$-balanced} (for $c \in [0, 1]$) if, for any $\allocs \in \polytope_{\matroid}$, each $i \in U$ is in the output~$S$ with probability at least $c\alloci$.
A CRS is said to be \emph{oblivious} if the knowledge of $\allocs$ is irrelevant for its output.

\paragraph{Online Contention Resolution Schemes (OCRS)}
An Online Contention Resolution Scheme (OCRS) is essentially a CRS that works in an online fashion.
It takes as input $\allocs \in \polytope_\matroid$, and sees the membership in~$R(\allocs)$ of the elements in~$U$ arriving in order;
when each element $i \in U$ arrives, if it is active (i.e., $i \in R(\allocs)$), the OCRS must decide irrevocably whether to include $i$ in its output~$S$.  
Like a CRS, the output~$S$ must always be an independent set in~$\matroid$.
The arrival order is called \emph{random} if it is uniformly at random, and the OCRS is called a \emph{random order OCRS} (RCRS);
the order is \emph{adversarial} if it is chosen by an adversarial who does not know $R(\allocs)$ (but knows $\allocs$);
the adversarial is \emph{almighty} if he knows $R(\allocs)$.
By default, in this paper, an OCRS works with an adversarial order. 
Without loss of generality, we assume the elements arrive in the order $1, 2, \ldots, n$.

Parallel to definitions for CRS, an OCRS is said to be \emph{$c$-selectable} (for $c \in [0, 1]$) if, for any $\allocs \in \polytope_{\matroid}$,  each element $i \in U$ is in the output~$S$ with probability at least $c \alloci$.
An OCRS is \emph{oblivious} if the knowledge of~$\allocs$ is irrelevant for its output.

\paragraph{(Matroid) Prophet Inequalities.}
In the matroid prophet inequality problem, we are given again a matroid $\matroid = (U, \indset)$, and for each $i \in U$, a distribution $\disti$. 
As each element arrives, a value $\vali$ independently drawn from~$\disti$ is revealed to the algorithm, and an irrevocable decision must be made whether to accept the element.
The algorithm should maximize the (expected) total value of accepted elements, while keeping the set of accepted elements independent in the matroid.
A prophet inequality algorithm is $c$-competitive (for $c \in [0, 1]$) if its expected value is at least $c$ fraction of the offline optimal, $\Ex{\max_{T \in \indset} \sum_{i \in T} \vali}$.
Prophet inequality is one of the best known applications of OCRS.  
A $c$-selectable OCRS algorithm immediately implies a $c$-competitive prophet inequality algorithm under the same arrival model \citep{FSZ16}.
\citet{LS18} showed that the converse is partially true: a prophet inequality algorithm that is $c$-competitive against the more powerful \emph{ex ante} optimal implies a $c$-selectable OCRS under the same arrival model.
\citet{KW19}'s matroid prophet inequality algorithm can be shown to be 2-competitive against the ex ante optimal, and it follows that a 2-selectable OCRS exists.

\paragraph{Laminar Matroids.}
A set family $\mathcal{L}\subseteq 2^U$ is \emph{laminar} if for any $A,B \in \mathcal{L}$, either $A \cap B = \emptyset$, or $A \subseteq B$ or $B \subseteq A$. 
A \emph{laminar matroid} is defined by a laminar family $\mathcal{L}$ and a set of positive integers $\{r_L\}_{L\in \mathcal{L}}$; a set $A\subseteq U$ is independent if and only if $|A\cap L|\leq r_L$ for all $L \in \mathcal{L}$. 
Without loss of generality, we may assume $r_L \leq |L|$ for every $L \in \mathcal L$, and $r_L < r_M$ for every $L$ that is a proper subset of $M$.
The polytope of a laminar matroid defined by the laminar family $\mathcal{L}$ and values $\{r_L\}_{L\in \mathcal{L}}$ is
$\mathcal{P}=\{\allocs\in [0,1]^U \ : \ \sum_{i\in L} x_i \leq r_L, \ \forall L\in \mathcal{L}\}$.




==> prophet.tex <==
%\subsection{Matroid prohpet inequality with \texorpdfstring{$O(\log n)$}{O(logn)} samples}
\subsection{Matroid prophet inequality with $O(\log n)$ samples}

\label{subsec:prophet}

Recall that we use $\matroid = (U, \indset)$ to denote a matroid, and for each item $i \in U$, its value $\vali$ is drawn independently from $\disti$. For simplicity, we shall assume that all $F_i$'s are continuous distributions. For general distributions with point masses, a standard tie-breaking technique can be applied. For completeness, we include it in Appendix \ref{appendix:point_mass}. 

We will need the strong basis exchange property for matroids throughout this section. Hence we include it here for completeness. 

\begin{lemma}[Strong basis exchange, Theorem 39.12 in \cite{schrijver2003combinatorial}] \label{lemma:strong_exchange}
	Let $\matroid = (U, \indset)$ be a matroid. Let $A$ and $B$ be two bases and $x \in A \setminus B$. Then there exists $y \in B \setminus A$ such that $A - x + y$ and $B - y + x$ are both bases.
\end{lemma}

We first give a few useful notations that shall be used in this subsection. %to compute the desired thresholds $\{T_k^i\}_{i \in [n], k \in [N]}$.
Given the realization of values $\vals$, we define $\OPT(\vals) \eqdef \max_{T \in \indset} \sum_{j \in T} \vali[j]$ to be the value of the maximum independent set and $\OPT_{i}(\valsmi) \eqdef \max_{T \in \indset, i \notin T} \sum_{j \in T} \vali[j]$ to the optimal value when item $i$ is removed. We assume w.l.o.g. that every $\OPT_i(\valsmi)$ is a basis. We can always add dummy elements with zero value to ensure it. For simplicity of notation, we omit $\vals$ when there is no obfuscation and abuse $\opt, \opt_{i}$ to denote the both optimal sets of items and their total values. 

Given $\valsmi$, define $\tau_i$ to be the smallest value among the items in $\OPT_{i}$ that $i$ can exchange with.
That is to say, $\tau_i(\valsmi) \eqdef \min\{\vali[j] \mid \OPT_{i} - j + i \in \indset \}$. 
Again, we omit $\valsmi$ when it is clear from the context.
%In particular, $\tau_i$ is the minimum value for $i$ to stay in the optimal basis, and the value of $\tau_i$ is independent of $\vali$. Moreover, if the minimum is attained at $j^*$, exchange $i$ into $\OPT_{(i)}$ results in a new set $\OPT_{(i)} - j^* + i$ with total value $\OPT_{(i)} - \tau_i + v_i$. 

%Then we show $\tau_i$ acts like a threshold indicating whether $i \in \OPT$ by the following fact.
The following observations regarding $\tau_i$ are useful in our later analysis.
\begin{observation}
\label{obs:is_threshold}
Fixing $\valsmi$, if $\vali > \tau_i(\valsmi)$, $i \in \opt(\vals)$; if $\vali < \tau_i(\valsmi)$, $i \notin \opt(\vals)$\footnote{We ignore the equality case which happens with zero probability.}.
\end{observation}
\begin{proof}
Let $j$ be the item whose value equals $\tau_i$. In the case when $\vali > \tau_i$, consider exchanging $i$ with $j$ in $\OPT_{i}$. This results in a basis of value $\OPT_{i} - \tau_i + \vali > \OPT_{i}$. Hence $\OPT_{i}$ is not optimal, and consequently $i \in \OPT$. 

For the other direction, we prove by contradiction. Suppose $i \in \OPT$, by Lemma \ref{lemma:strong_exchange}, there is an element $j \in \OPT_i$ such that $\OPT - i + j$ and $\OPT_i - j + i$ are both bases. Since $\OPT - i + j \in \indset$, by optimality of $\OPT$, $v_j \leq v_i$. Moreover, since $\OPT_i - j + i \in \indset$, by the definition of $\tau_i$, we have $\tau_i \leq v_j$. Hence $\tau_i > v_j$ implies $i \not\in \OPT$.
%\zhihao{The other direction does not follow the same argument. Please help complete the proof. And where do we use the two observations? In Lemma~\ref{lemma:threshold_concentration}? }    
%\Hongxun{Added. Yes we use them there.}
\end{proof}

\begin{observation}
\label{obs:tau_property}
Suppose $i \in \OPT$, $j \notin \OPT$ and $\OPT- i + j \in \indset$. Then $\vali \ge \tau_j$.
\end{observation}
\begin{proof}
Since $j \not\in \OPT$, we have $\OPT_j = \OPT$. Together with the fact that $\OPT - i + j$ is also an independent set, we have $\tau_j \leq \vali$ (by the definition of $\tau_j$). 
\end{proof}


Our algorithm contains two stages. In the first stage, we estimate the thresholds $\{T_k^i\}$ from $O(\log n)$ samples. In the second stage, we learn an OCRS from another $O(\log n)$ samples. We first present the first stage. Let $m = \lfloor \log_{1 + \epsilon}(1/\epsilon) \rfloor$.

%Let $m = \lfloor \log_{1 + \epsilon}(1/\epsilon) \rfloor$.
%However, without explicit knowledge of $\disttaui$, we can only estimate $\tau_i$ by samples from $\disttaui$, which can be further obtained by samples from $\dist$. In order to roughly recover $\disttaui$, here we estimate $K=\lfloor\log_{1+\epsilon}(1/\epsilon)\rfloor$ many quantiles of it. The $k$-th quantile $T_{i,k}$ approximates $\disttaui^{-1}(\epsilon(1+\epsilon)^k)$. They are estimated using $N$ samples from $\dist$ as described in Algorithm \ref{alg:prophet_threshold}.

\paragraph{Learning Thresholds.} Given $N$ i.i.d. samples $\vals^s \sim \times_{i} F_i$, where $s \in [N]$.
For each item $i$, let $T_k^i$ be the $\lceil\epsilon(1+\epsilon)^kN\rceil$-th smallest value in $\{\tau_i(\valsmi^s) \mid s \in [N]\}$ for $0\le k< m$ and $T_m^i = \infty$.

%\begin{algorithm}[H]
%\SetAlgoLined
%  \For{$s \gets 1,2,...,N$}{
%    {Sample a new set of values $\{\vali^s \mid i \in U\}$, where $\vali^s$ is drawn from $\disti$}\\
%    \For{$i \in U$}{
%      {$\tau_{i}^s \gets \min\{\vali[j]^s \mid \OPT^s_{(i)} - j + i \in \indset \}$}
%    }
%  }
%  
%  {$K \gets \lfloor \log_{1 + \epsilon}(1/\epsilon) \rfloor$}
% 
%  \For{$i \in U$}{
%    \For{$k \gets 0,1,...,K-1$}{
%      {$T_{i,k} \gets$ the $\lceil\epsilon(1+\epsilon)^kN\rceil$-th smallest value in $\{\tau_i^s \mid 1 \le s \le N\}$}
%    }
%    {$T_{i,K} \gets \infty$}
%  }
%\caption{Estimating all thresholds $T_{i,k}$ with $N$ samples}
%\label{alg:prophet_threshold}
%\end{algorithm}

%\begin{observation}
%In Algorithm \ref{alg:prophet_threshold}, for each $i \in U$, $\tau_i^1, \tau_i^2, \dots, \tau_i^N$ are i.i.d. random variables each distributed according to CDF $\disttaui$. 
%\end{observation}

%Then we take $N=\Theta(\log n)$ samples, and formally show all $T_{i,k}$ can approximate $\disttaui^{-1}(\epsilon(1+\epsilon)^k)$ simultaneously with high probability. 
The next lemma states that the thresholds $\{T_k^i\}$ approximates the functions $p^i(v) \eqdef \Prx{i \in \opt \mid v_i=v}$ within $\epsilon$ accuracy. The proof is a direct application of Chernoff bound and we defer it to Appendix \ref{appendix:threshold_concentration}.
Let $p_k = \epsilon(1+\epsilon)^k -\epsilon^2$ for $0 \le k < m$. Note by Observation \ref{obs:is_threshold}, we have $p^i(v) = \Pr[v > \tau_i]$ for any fixed $v$, and $\{T_k^i\}$ are fixed values (not random variables) here. 

\begin{lemma} \label{lemma:threshold_concentration}
For any $\epsilon \in (0,1)$, with $N=O(\log(\frac{2nm}{\epsilon}) \cdot \epsilon^{-4})$ samples, $p^i(T_{k}^i) = \Pr[T_{k}^i > \tau_i] \in [p_k,p_k+2\epsilon^2]$ for all $i \in U$ and $0 \le k < m$ with probability at least $1 - \epsilon$. We refer to such thresholds as \emph{good} thresholds.
\end{lemma}

Once we have estimated these thresholds, we view them as fixed value rather than random variables (i.e. conditioning on the value of these thresholds). This is important for the independence required by OCRS. 

%\Hongxun{TODO: Here we prove it for $p^i(T_k^i)$ which is different with $G_i(T_k^i)$. We need to rewrite appendix, and use Observation \ref{obs:is_threshold} to prove they are equal. }

\paragraph{Activation Rule.} With these thresholds, we specify a rule of determining whether an item $i$ is active. If $v_i \in [T_k^i, T_{k+1}^i)$ for some $ 0\le k<m$, let $i$ be active with probability $p_k$; else $v_i \in [0, T_0^i)$, let $i$ be active with probability $0$.
Let $\alloci = \Prx{i \text{ is active}}$, where the probability space only involves randomness of $v_i \sim F_i$.

For any $\vals \sim \times_i F_i$, we can then apply this activation rule to each of the items to generate a set of active items. It is important that in this stage, we do not reuse the samples from the first stage. The reason is that there are correlations between the thresholds we learnt for different items, but OCRS requires each item to be active independently. Thus we treat the thresholds now as fixed values and use a new sample $\vals$ to generate a sample of $R(\allocs)$. Observe that in this way, each element is active independently. 

%Observe that in this way, each item is active independently. 
%Now we prove that the vector $\allocs \in \polytope_{\matroid}$ whenever the thresholds satisfy the conditions stated in Lemma~\ref{lemma:threshold_concentration}
\begin{lemma}
	\label{lemma:ocrs_validity}
	If $\{T_k^i\}$ are good thresholds, then $\allocs \in \polytope_{\matroid}$.
\end{lemma}

\begin{proof}
	Let $\alloci^*=\Prx{i \in \OPT}$ for every $i \in U$. Since $\OPT \in \indset$, we have $\allocs^* \in \polytope_{\matroid}$. Consider the conditional probability of $i$ being active when $\vali = v$.
	\begin{itemize}
	\item If $v<T_0^i$, $\Prx{i \text{ is active} \mid v_i=v} = 0 \le p^i(v)$. 
	\item If $v \in [T_{k}^i, T_{k+1}^i)$ for $0\le k <m$, we have 
	\[
	\Prx{i \text{ is active} \mid \vali=v} = p_k \le p^i(T_k^i) \le p^i(v),
	\]
	where the first inequality follows from the assumption of $T_i^k$ and the second inequality follows from the monotonicity of function $p^i$.
	\end{itemize}
	Therefore, for each $i\in U$,
	\[
	\alloci = \int_v \Prx{i \text{ is active} \mid \vali = v} \dd F_i(v) \le \int_v p^i(v) \dd F_i(v) = \alloci^*,
	\]
	that concludes the proof of the lemma.
\end{proof}

Furthermore, the expected values of active items are large compared to the expected optimal. This is the most technical lemma and the proof is built on a novel monotone basis exchange lemma for matorids, that might be of independent interests. We defer the proof to Subsection~\ref{subsec:bases_exchange}.
\begin{lemma}
	\label{lemma:prophet_competitive_ratio}
	If $\{T_k^i\}$ are good thresholds, then $\E{\sum_{i \in R(\allocs)} v_i} \ge (1-O(\epsilon)) \cdot \E{\opt}$.
\end{lemma}
%Having estimated these values using Algorithm \ref{alg:prophet_threshold} with $N=3\log(2Kn/\epsilon)/\epsilon^4$, we can transform the original problem into an OCRS problem with the same matroid constraint $\matroid = (U,\indset)$. Recall that $R$ is the random set of active elements. When item $i$ arrives with value $v_i$, we let it be active with the following probability:
%\begin{equation*}
%    \Prx{i \in R \mid \vali=t} =
%    \begin{cases}
%        \epsilon(1+\epsilon)^k-\epsilon^2, & \exists\ 0 \le k < K,\ t \in [T_{i,k},T_{i,k+1})\\
%        0, & 0 < t < T_{i,0}
%    \end{cases}
%\end{equation*}
%
%\begin{observation}[Informal version of Lemma \ref{lemma:ocrs_validity}, (1)] \label{obs:indpednent}
%Given thresholds $\{T_{i,k}\}$, for each $i, j \in U$, $i \not= j$, $i \in R$ and $j \in R$ are independent events. 
%\end{observation}
%
%The probability for item $i$ to be active is $\alloci = \Prx{i \in R}=\int_0^\infty \Prx{i \in R \mid \vali=t}\ \mathrm{d} F_i(t)$.
%We will show $\allocs \in \polytope_\matroid$, so together with Observation \ref{obs:indpednent}, $R$ is a valid input for OCRS.
%
%However, $\allocs$ is unknown to the algorithm since the distribution $F_i$ is unknown. Thus we need OCRS from $O(\log n)$ samples. Having defined these probabilities, a sample from $R$ can be precisely generated from an extra sample \footnote{In order for Observation \ref{obs:indpednent} to hold, it is important that we do not reuse the samples in Algorithm \ref{alg:prophet_threshold}.} of $\vals$. Our algorithm then follows by directly applying the $(1/4-\epsilon)$-selectable OCRS from Theorem \ref{thm:matroid_ocrs}.
%In order to make our algorithm always stops, it terminates if the chain construction of OCRS is stuck at some layer (see \Qianfan{TODO: appendix} for details).It also terminates if the OCRS subroutine attempts to select an element violating matroid constraint.
%\begin{observation}\label{obs:prophet_correctness} The algorithm never selects an infeasible set of elements and always terminates. \end{observation}

%\begin{algorithm}[H]
%\SetAlgoLined
%{\emph{Prepare stage}}\\
%{$K \gets \lfloor \log_{1+\epsilon}(1/\epsilon) \rfloor$}\\
%  {Call Algorithm \ref{alg:prophet_threshold} with $N=3\log(2Kn/\epsilon)/\epsilon^4$ to estimate all thresholds $T_{i,k}$}\\
%  {Construct matroid OCRS with $O(\log n)$ samples}\\
%{\emph{Running stage}}\\
%  {Apply matroid OCRS}
%\caption{$(4+\epsilon)$-competitive algorithm for matroid prophet inequality with $O(\log n)$ samples}
%\label{alg:prophet}
%\end{algorithm}

%\subsubsection{Analysis}

%\Qianfan{The proof here is ugly and might be simplified.} \Hongxun{Yes it can be. Now it's one-line lovely proof.}

%\begin{proof} Suppose we have such $i,j$ and $\vali < \tau_j$. Consider another realization $\val'$ where $\vali[j]'=(\vali+\tau_j)/2$ and $\vali[k]'=\vali[k]$ for every $k \in U-\{j\}$, so that $\vali' < \vali[j]' < \tau_j$. Define $\OPT'$ and $\tau'$ correspondingly and we have $\tau_j'=\tau_j$ by definition. But $\vali[j]' < \tau_j = \tau_j'$ implies $j \notin \OPT'$. Therefore $\OPT$ is still an optimal basis with respect to $\val'$, contradicting with $\OPT-\{i\}+\{j\} \in \indset$ and $\vali[j]'> \vali'$. \end{proof}

Now, we have all the components to prove our main theorem.
\begin{theorem}\label{thm:matroid_prophet}
With $\tilde{O}(\log n)$ samples\footnote{The $\tilde{O}$ notation hides all factors related to $\epsilon$.}, there is a $(\frac{1}{4}-\epsilon)$-competitive algorithm for the sample-based matroid prophet inequality problem.
\end{theorem}

\begin{proof}
We first use $\tilde{O}(\log n)$ samples to learn the thresholds $\{T_k^i\}$. By Lemma~\ref{lemma:threshold_concentration} and Lemma~\ref{lemma:ocrs_validity}, the thresholds are good with at least $(1-\epsilon)$ probability and the corresponding activation rule results in a valid $\allocs \in \polytope_{\matroid}$.
We then use another $\tilde{O}(\log n)$ samples to learn the corresponding $(\frac{1}{4}-\epsilon)$-selectable OCRS $A$ by Theorem~\ref{thm:matroid_ocrs}.
Finally, in the real run of the prophet inequality, upon the arrival of an item $i$, we use the activation rule constructed above to decide whether $i$ active and feed it to the OCRS $A$.
	
Let $\ALG$ be the random set of elements selected by the algorithm. Let $\event$ be the event that $\{T_k^i\}$ are good thresholds. 
\begin{align*}
\E{\sum_{i \in \ALG} \vali} \ge{} & \Prx{\event} \cdot \operatorname{\mathbf E}\left[ \sum_{i\in \ALG} \vali \;\middle|\; \event \right] \\
\ge{} & (1-\epsilon) \cdot \left(\frac{1}{4} - \epsilon\right) \operatorname{\mathbf E}\left[ \sum_{i\in R(\allocs)}\vali \;\middle|\; \event \right] & \mbox{by Lemma~\ref{lemma:threshold_concentration} and Theorem~\ref{thm:matroid_ocrs}} \\
\ge{} & (1-\epsilon) \cdot \left(\frac{1}{4} - \epsilon \right) \cdot \left(1-O(\epsilon) \right) \cdot \E{\opt} & \mbox{by Lemma~\ref{lemma:prophet_competitive_ratio}} \\
={} & \left(\frac{1}{4}-O(\epsilon)\right) \cdot \E{\opt},
\end{align*}
that concludes the proof of the theorem.
\end{proof}

